Raman Scattered HeII 6545 in the Young and Compact Planetary Nebula NGC 6790

We present the high resolution spectra of the youn and compact planerary nebula NGC 6790 obtained with the echelle spectrograph at Bohyunsan Optical Astronomy Observatory and report the discovery of Raman scattered He II 6545 in this object. This line feature is formed in a thick neutral region surrounding the hot central star, where He II 1025 line photons are scattered inelastically by hydrogen atoms. A Monte Carlo technique is adopted to compute the line profile with a simple geometric model, in which the neutral region is in the form of a cylindrical shell that is expanding from the central star. From our line profile analysis, the expansion velocity of the HI region lies in the range V_exp = 15- 19 Km/s. Less stringent constraints are put on the HI column density N_HI and covering factor C, where the total flux of Raman He II 6545 is consistent with the product of N_HI and C being CN_HI ~ 0.5 X 10^20 cm^-2. The Monte Carlo profiles from stationary emission models exhibit deficit in the wing parts. A much better fit is obtained when the He II emission region is assumed to take the form of a ring that slowly rotates with a rotation speed ~ 18Km/s. Brief discussions are presented regarding the mass loss processes and future observations.

==> cover1 <==

Dear Editor,

We uploaded a revised version of our paper
'Raman Scattered He II 6545 in the Young and Compact Planetary
Nebula NGC 6790"'
by Eun-Ha Kang, Byeong-Cheol Lee and Hee-Won Lee.
The revision was made by respecting  all the suggestions made by the
referee, to whom we are very grateful for his/her constructive comments.
Mainly there were 6 quries (suggestions) made by the referee.


The following are the answers to the requests of the referee.

1. We have a strong doubt that Aller et al.(1996) would have noticed the existence of Raman 6545 feature in their spectrum of NGC 6790 because Raman 6545 appears at most as a broad wing around [N II] 6548. 
Perhaps in their spectrum there appeared a weak narrow emission line around at 6545, but in our spectra we can only notice a broad feature centered at 6547, and no discernible emssion line at 6545.

2. The unidentified emission line that appears at 6528 is not [N II] 6527. 
According to NIST data, [N II] 6527 has a center wavelength at 6527.23 with the Einstein coefficient A = 5.45x10^{-7} s^{-1}. 
Compared with [N II] 6548 which has a center wavelength at 6548.05 \AA\ with A = 9.19x10^{-4}, [N II] 6527 is weaker than [N II] 6548 by a factor of 1700.
Based on these atomic data, we plotted [N II] 6527 with a dot-dashed line is 
fig2.  As is shown in the figure [N II]6527 is significantly weaker 
than He II 6527, and hence can not affect the over all line fitting result.
The 6528 feature is much stronger than [N II] 6527 and still remains 
to be identified.

We didn't bother to derive the heliocentric systematic velocity.
And NIST data were essential to de-blend the complex feature of (He II 6527 + unidentified line).
However we re-wrote the sentence about NIST.
We also added the statement that Th-Ar lamp was used for wavelength calibrations in the 1st paragraph in section 2.1.

3. OK.
We also added a figure showing the expected Raman He II 4850 around H$\beta$.

4. We didn't find suitable UV data from HUT and FUSE. We mentioned this 
in section 3.2.2.

5. We normalize the flux by [N II] 6548, which is set to have a flux 
density peak of unity. In this way, all the other emission lines can 
be more easily compared with each other.

6. We opted the current approach because of the strong blending and the additional absorption feature in [N II] 6548.
We add a new paragraph to this effect in the last part of section 2.2.

-----------------------

The following is the change of the manuscript in the revised version.

1. In the abstract, 
'with the product of N_HI and C' --> 'with their product CN_HI'

2. In the first paragraph of section 2.1 we added a sentence
'A Th-Ar lamp was used for wavelength calibrations.'

3. In the second paragraph of section 2.1 we added two sentences
explaining the normalization of the flux appearing in the vertical axis.
This answers query 5 by the referee.

'The vertical axis represents the relative flux density.
We normalize the flux density using [N~II]$\lambda$6548, which is set 
to have a flux density peak of unity.'

4. In the first paragraph of section 2.2, we re-wrote statements related
with the wavelength difference and atomic data of NIST. 

In the current version, the new statements are
'We use the atomic spectral data from the website of the National 
Institute of Standard and Technology(NIST), from which we note 
that each emission line in our spectra of NGC~6790 appears systematically 
redward of atomic line center by an amount of 20.7${\rm\ km\ s^{-1}}$.'

5. In the last part of section 2.1, we changed our conclusion about
Raman scattered He II 4850, as is suggest by the referee (Query 3).

6. In section 2.2 before Eq.1, we added our analysis of [N II}6527, as
is suggested by the referee. The following has been added in the revised
version. 

'Groves et al.(2002) noted the existence of [N II]$\lambda$6527
redward of He II$\lambda$6527 with the wavelength difference of 0.14 \AA\
in their spectrum of NGC 6302. However, the unidentified emission line 
in our spectrum of NGC 6790 can not be [N II]$\lambda$6527, because 
it appears redward of He~II$\lambda$6527 by 1 \AA. Furthermore, based on 
the NIST data, [N II]$\lambda$6527 has the Einstein A coefficient 
$A =  5.45\times 10^{-7} s^{-1}$. Compared with [N II]$\lambda$6548 
having $A = 9.19\times 10^{-4}$, [N II]$\lambda$6527 should be 
weaker than [N II]$\lambda$6548 by a factor of 1700.
Based on these atomic data, we plotted [N~II]$\lambda$6527 
with a dot-dashed line in Fig.2.
As is shown in the figures, [N II]$\lambda$6527 is significantly weaker 
than He~II$\lambda$6527, and hence can not affect the over all line 
fitting result.
The 6528\AA feature is much stronger than [N II]$\lambda$6527 and still 
remains to be identified.'


7. In the last part of section 2.2 we added a following new paragraph 
related with query 6 by the referee.

' Lee, Kang \& Byun(2001) performed a line profile analysis of Raman scattered 
He~II$\lambda$6545 in a number of symbiotic stars. They subtracted one third 
of the flux near [N II]$\lambda$6583 from the flux near [N~II]$\lambda$6548 
to expose a broad Raman scattering line feature successfully.
However, in view of the existence of the unidentified absorption feature 
in [N~II]$\lambda$6548 and more severe blending with [N~II]$\lambda$6548, 
we took another approach, in which the Raman scattered He~II$\lambda$6545 
feature is directly fitted from our Monte Carlo data.'


8. In the last part of subsection 3.2.1, we added a following new paragraph
in accordance with suggestion 3 by the referee.


'Jung \& Lee (2004b) developed a Monte Carlo code to compute
the line profile of Raman scattered He~II 4850 and analyzed
their spectrum of the symbiotic star V1016~Cyg.
Using the same code, we show in Fig.~7 the Monte Carlo profile
for Raman scattered He~II 4850 by a long dashed line. The same
column density and covering factor as in Fig.~6 were used in this
calculation. In the figure, the solid line shows the BOES data with
the exposure time of 7200 s. Our observational data are barely
consistent with our interpretation of Raman scattering nature.
The poor quality of the current observational data hinders a further
serious quantitative analysis. A more fruitful analysis may
be made only after observational data with a better quality
are secured.'

9. The following sentence was added in the second paragraph 
of subsection 3.2.2 in accordance with query 4 by the referee.

'No observational data of NGC~6790 are available in the archives of
HUT and FUSE.'


10. In the caption of Fig.1, we added a sentence explaining the normalization
of relative flux. This change is made in accordance with Query 5 by the
referee.

11. In the caption of Fig.2, a sentence on the flux normalization is added.

12. In panel (c) of Fig. 2, we added a emission line component [N II]6527
by a dot-dash line. The caption was also changed appropriately with this
addition of [N II]6527. This change is in accordance with Query 2 by the
referee. 

13. We added a new figure (Fig. 7) showing Raman scattered He 4850,
which is suggested by the referee (Query 3).

